A Spectral Framework for Tracking Communities in Evolving Networks

Discovering and tracking communities in time-varying networks is an important task in network science, motivated by applications in fields ranging from neuroscience to sociology. In this work, we characterize the celebrated family of spectral methods for static clustering in terms of the low-rank approximation of high-dimensional node embeddings. From this perspective, it becomes natural to view the evolving community detection problem as one of subspace tracking on the Grassmann manifold. While the resulting optimization problem is nonconvex, we adopt a block majorize-minimize Riemannian optimization scheme to learn the Grassmann geodesic which best fits the data. Our framework generalizes any static spectral community detection approach and leads to algorithms achieving favorable performance on synthetic and real temporal networks, including those that are weighted, signed, directed, mixed-membership, multiview, hierarchical, cocommunity-structured, bipartite, or some combination thereof. We demonstrate how to specifically cast a wide variety of methods into our framework, and demonstrate greatly improved dynamic community detection results in all cases.

==> 2_proposed-framework/taxonomy-table.tex <==
\jake{I wonder if the `assignments via' should be traded for less acronyms... }
\begin{table}[h]
\caption{ \textcolor{orange}{this is back to a WIP \textit{would this be better formatting as 'network type', 'algorithm/matrix', 'example application'}?} Taxonomy of spectral algorithms for static graph community detection. Included are SGP (spectral graph partitioning) , USC (unnormalized spectral clustering), NSSC (normalized symmetric spectral clustering), SMM (spectral modularity maximization, where $\langle A \rangle$ denotes the Newman-Girvan null model average adjacency matrix $A_{ij}={\operatorname{deg}(i)\operatorname{deg}(j)}/{\operatorname{vol}(A)}$), SSC (signed spectral clustering), OSC (overlapping spectral clustering), and DSC (directed spectral clustering, where $\boldsymbol M \big(\operatorname{sym}(\boldsymbol A)\big)$ denotes a clustering matrix obtained via some symmetrization of $\bs A$). VP abbreviates \textit{vector partitioning}.} 
\centering
\renewcommand{\arraystretch}{1.5}  % Slightly increase overall row height
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Algorithm} & \textbf{Clustering Matrix $\bs M$} & \textbf{Assignments via...}& \textbf{Example Application} \\
\hline
SGP \cite{alpert_spectral_1995}& $\displaystyle \overline{\boldsymbol L}=\boldsymbol I-\frac{\boldsymbol D - \boldsymbol A}{2n}$ & Size-constrained VP& Circuit partitioning \cite{alpert_recent_1995} \\[6pt]
\hline
USC \cite{belkin_laplacian_2003} & $\displaystyle \overline{\boldsymbol L}=\boldsymbol I-\frac{\boldsymbol D- \boldsymbol A}{2n}$ & $k$-means & Manifold learning  \cite{belkin_laplacian_2003} \\[6pt]
\hline
NSSC \cite{ng_spectral_2001} & $\displaystyle \boldsymbol Q^{\text{sym}}=\boldsymbol D^{-\frac{1}{2}}(\boldsymbol D + \boldsymbol{A}) \boldsymbol D^{-\frac{1}{2}}$ & $k$-means & Image segmentation \cite{shi_normalized_2000}\\[6pt]
\hline
%WS-MM & $\displaystyle \widetilde{\boldsymbol B} = \boldsymbol D ^{-1} \boldsymbol A$ & $k$-means & [TODO] \\[6pt]
%\hline
MM \cite{white_spectral_2005} & $\widehat{\boldsymbol{B}} = \bs I + \frac{\bs A - \langle \bs A \rangle}{\|\bs A - \langle \bs A \rangle\|_{\text{F}}}$& $k$-means & Brain connectivity \cite{bullmore_complex_2009}\\[6pt]
\hline
 SSC \cite{mercado_pedro_pdf_nodate} & $\overline{\bs L}(p)=\boldsymbol I-  \frac{1}{2} \bs M_{p}(\boldsymbol L^{\text{sym}+}, \boldsymbol Q^{\text{sym}-})$ & $k$-means& Time series \cite{aghabozorgi_time-series_2015}  \\ \hline
 OSC \cite{scott_wahl_hierarchical_nodate}& $\displaystyle \boldsymbol Q^{\text{sym}}=\boldsymbol D^{-\frac{1}{2}}\boldsymbol (\boldsymbol{D} + \boldsymbol{A}) \boldsymbol D^{-\frac{1}{2}}$& Fuzzy $c$-means& Social networks \cite{devi_analysis_2016} \\\hline
 DSC \cite{satuluri_symmetrizations_2011} & $\boldsymbol M \big(\text{sym}(\boldsymbol A)\big)$& Variable&Genomics \cite{popa_directed_2011} \\\hline
\end{tabular}
\label{tab:spectral-algorithms}
\end{table}



==> 4_backmatter/author-contributions.tex <==
\jake{TODO (I don't know what to put here) (doesn't count toward page limit)}
